Regional and Temporal Patterns of Partisan Polarization during the COVID-19 Pandemic in the United States and Canada

Public health measures were among the most polarizing topics debated online during the COVID-19 pandemic. Much of the discussion surrounded specific events, such as when and which particular interventions came into practise. In this work, we develop and apply an approach to measure subnational and event-driven variation of partisan polarization and explore how these dynamics varied both across and within countries. We apply our measure to a dataset of over 50 million tweets posted during late 2020, a salient period of polarizing discourse in the early phase of the pandemic. In particular, we examine regional variations in both the United States and Canada, focusing on three specific health interventions: lockdowns, masks, and vaccines. We find that more politically conservative regions had higher levels of partisan polarization in both countries, especially in the US where a strong negative correlation exists between regional vaccination rates and degree of polarization in vaccine related discussions. We then analyze the timing, context, and profile of spikes in polarization, linking them to specific events discussed on social media across different regions in both countries. These typically last only a few days in duration, suggesting that online discussions reflect and could even drive changes in public opinion, which in the context of pandemic response impacts public health outcomes across different regions and over time.

==> 024_R4.tex <==

 


\subsection{The Relationship between Conspiracy and Polarization}

%We observed that particular conspiracy tweets and narratives coincided with periods of intense political discussions and high polarization, which are likely fueled by these widespread conspiracy theories and misinformation. We discussed the polarization peaks in more details in the earlier section. 
Here, to confirm the overall relationship, we look into the correlation between the polarization and volume of the conspiracy related tweets posted daily.  Although some peaks correlated, interestingly, Figure \ref{fig:cad_political_aggregated_corr} suggests that overall \textit{conspiracy tweet volume is negatively correlated with polarization in Canada}. This might be explained by the decline of conspiracy related content and debunking of misinformation as more scientific evidence is provided overtime, as well as the rise in the polarization as the severity of the pandemic increased, as seen in Figure \ref{fig:aggregated_corr_polarization_and_conspiracy}. 

% We want to highlight that although higher volume of conspiracy is posted by the right party family, there is strong negative correlations between partisan polarization and conspiracy posted from the users in both the left and the right party families. 
% In particular, while the correlation is \textbf{-0.62} for the overall volume, which sums the two, as reported in Figure \ref{fig:cad_political_aggregated_corr}, we still observe a correlation of {-0.62} with CI = [-0.74, -0.48] (n = 88, p = 7.92e-11) for the volume of conspiracy related post from the left party family users; and interestingly, a lower correlation of {-0.56} CI = [-0.69, -0.40] (n = 88, p = 1.01e-08) with the volume of the conspiracy related posts from the right party family users.
% We want to highlight that there is also negative correlations within both the left and the right party families, which suggests the correlation is more complex. In particular, while the overall correlation is \textbf{-0.62} as reported in Figure \ref{fig:cad_political_aggregated_corr}, looking at only left or right party families, we still observe a correlation of \textbf{-0.62} with CI = [-0.74, -0.48] (n = 88, p = 7.92e-11),  for the left to \textbf{-0.56} (n = 88, p = 1.01e-08, CI = [-0.69, -0.40]) for the right.
% Figure \ref{fig:cad_political_consp_vol} confirms that the volume of conspiracy-related tweets per party coincides with periods of intense political discussions, marked by widespread conspiracy theories and misinformation in Canada \citep{XXXX}. For example, on Dec 10, 2020, we found several political discussions related to XXXXX. One prevalent claim was about a secret meeting happening to discuss the political relationship between Justin Trudeau and the Chinese Communist Party (CCP) during the pandemic. More on this.

The rise in the volume of conspiracy-related tweets coincides with periods of intense political discussions with varying amounts of polarization. Hence, we did not observe a significant correlation in the United States. On November \nth{16}, 2020, we find a clear peak with 18,082 tweets mainly related to the Great Reset \cite{schuller2021world} were found. The Great Reset refers to a UN Agenda initiative proposed to promote a more sustainable future. However, conspiracy theorists have turned it into a narrative of nefarious elites intentionally creating \COVID (such as ploy led by Prime Minister Justin Trudeau to take over the global economy) \citep{Goodman2020Carmichael}. Another interesting peak takes place on November \nth{21}, 2020, coinciding with the reach of more than 12 million coronavirus cases in the US \cite{Latif2020}.  On \textbf{November 28th, 2020}, some users were posting tweets arguing that Donald Trump was right to accuse the US 2020 presidential election of being rigged and that COVID-19 was part of the plan in stealing the election. For example, one user wrote: "@realDonaldTrump @OANN Do you think COVID-19 was part of the plan to try to steal an election, and it was created in China w…". On the same day, Trump expressed his doubt about whether the Supreme Court would acknowledge his allegations of fraud while the two largest counties in Wisconsin recounted ballot votes and certified Joe Biden as the winner \citep{Helderman-Gardner2020}. Another clear conspiracy peak is on December \nth{21}, 2020, when several political events related to \COVID occurred. First, Congress passed the \$900 billion coronavirus relief package \cite{jacob2020}. Second, Biden received his first vaccine dose live \cite{melissa2020}. Finally, a disruptive protest on reopening the state and removing lockdown measures occurred in front of Oregon's Capitol building \citep{oneil2020}. 

\begin{figure}[h!]
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[scale=0.43]{Daily Polarization/CAD_political/conspiracy.png}
        \caption{Volume of Conspiracy-related Tweets}
        \label{fig:cad_political_consp_vol}
    \end{subfigure}
    \hspace{0.01\linewidth}
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[scale=0.43]{Daily Polarization/CAD_political/unweighted_agg_poli_consp_vol.png}
        \caption{Polarization v.s. Conspiracy Volume}
        \label{fig:cad_political_aggregated_corr_consp}
    \end{subfigure}
    \\
     \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[scale=0.43]{Daily Polarization/US/conspiracy.png}
        \caption{}
        \label{fig:us_conspiracy_vol}
    \end{subfigure}
    \hspace{0.01\linewidth}
    \begin{subfigure}{0.48\linewidth}
        \centering
        \includegraphics[scale=0.43]{Daily Polarization/US/unweighted_agg_poli_consp_vol.png}
        \caption{}
        \label{fig:us_aggregated_corr_consp}
    \end{subfigure}
    \caption{Relation between the volume of conspiracy related content and the observed partisan polarization in the U.S. and Canada. 
    (a) for Canada, we report the volume of conspiracy related tweets posted by users from the Left Party Family (LPF)---Liberal, New Democratic Party, Green, and the Right Party Family (RPF)---Conservative, People's Party for Canada. For the U.S., we report the volume between Democrat and Republican users. 
    On the right, we show the relation between daily partisan polarisation summed over the different topics and the overall volume of conspiracy tweets. In Canada, we find that there is no statistically significant correlation of \textbf{0.023} with CI=[-0.187,0.231] (n = 88,  p=0.831) between these measures. In the U.S., we find there is a statistically significant correlation \textbf{-0.247} with CI=[-0.448,-0.023] (n = 88,  p=0.031) between these measures.}
    \label{fig:aggregated_corr_polarization_and_conspiracy}
\end{figure}

Finally, we note in Figure \ref{fig:US_AVG_WKLY_CONSP_POL} that the percentage of conspiracy-related tweets are higher in swing states (Arizona, Florida, Georgia, Michigan, Minnesota, North Carolina, Pennsylvania and Wisconsin). 

We also note that the volume of conspiracy-related tweets in the United States follows a general trend of decline during the period under study, which covers the 2020 presidential election and its aftermath.


%\subsection{Relationship between Vaccine Polarization and \COVID Epidemiology Data}



%\begin{figure}[h!]
%    \begin{subfigure}{0.48\linewidth}
%        \centering
%        \includegraphics[scale=0.43]{Daily Polarization/CAD_political/vaccine_COVID_cases.png}
%        \caption{Vaccine Polarization}
%        \label{fig:cad_political_vax_pol}
%    \end{subfigure}
%    \hspace{0.01\linewidth}
%    \begin{subfigure}{0.48\linewidth}
%        \centering
%        \includegraphics[scale=0.43]{Daily Polarization/CAD_political/vaccine_COVID_cases_corr.png}
%        \caption{Vaccine Polarization \& COVID-19 Deaths Correlation}
%        \label{fig:cad_political_vax_pol_covid_deaths_corr}
%    \end{subfigure}
%    \\
%     \begin{subfigure}{0.48\linewidth}
%        \centering
%        \includegraphics[scale=0.43]{Daily Polarization/US/vaccine_COVID_cases.png}
%        \caption{Vaccine Polarization}
%        \label{fig:us_vax_pol}
%    \end{subfigure}
%    \hspace{0.01\linewidth}
%    \begin{subfigure}{0.48\linewidth}
%        \centering
%        \includegraphics[scale=0.43]{Daily Polarization/US/vaccine_COVID_cases_corr.png}
%        \caption{Vaccine Polarization \& COVID-19 New Cases Correlation}
%        \label{fig:us_vax_pol_covid_cases_corr}
%    \end{subfigure}
%    \caption{Relation between the observed vaccine partisan polarization and \COVID epidemiology data in Canada and the United States. On the left, we report the vaccine partisan polarization. On the right, we show the relation between daily vaccine polarization and the most correlated \COVID epidemiology data. We find that in Canada, there is a correlation of \textbf{0.361} with CI = [0.164, 0.530] (n = 88,  p = 0.001) between these measures. For the United States, we also observe a correlation of \textbf{-0.246} with CI = [-0.446, -0.021] (n = 79, p = 0.033).}
%    \label{fig:vax_pol_and_covid_corr}
%\end{figure}





==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
